Self-supervised Pretraining for Partial Differential Equations

In this work, we describe a novel approach to building a neural PDE solver leveraging recent advances in transformer based neural network architectures. Our model can provide solutions for different values of PDE parameters without any need for retraining the network. The training is carried out in a self-supervised manner, similar to pretraining approaches applied in language and vision tasks. We hypothesize that the model is in effect learning a family of operators (for multiple parameters) mapping the initial condition to the solution of the PDE at any future time step t. We compare this approach with the Fourier Neural Operator (FNO), and demonstrate that it can generalize over the space of PDE parameters, despite having a higher prediction error for individual parameter values compared to the FNO. We show that performance on a specific parameter can be improved by finetuning the model with very small amounts of data. We also demonstrate that the model scales with data as well as model size.

==> src/experiments/tables/channels.tex <==
% \vspace{0.2cm}
% Test results for trajectories (unseen during training) with $\theta \in \theta_{pt}$ (seen parameters) after pre-training but before finetuning with increasing model size.

% \vspace{0.2cm}
% \begin{tabular}{>{\centering\arraybackslash}p{0.10\linewidth}|>{\centering\arraybackslash}p{0.12\linewidth}|>{\centering\arraybackslash}p{0.12\linewidth}|>{\centering\arraybackslash}p{0.12\linewidth}|>{\centering\arraybackslash}p{0.12\linewidth}}
%     \hline
%     $\theta$ & $traj$     & $traj + t$ & $traj + t + param$ & $traj + t + param + fft$ \\
%     \hline
%     0.001    & 0.007389 & 0.010944 & 0.003404         & 0.005982               \\
%     0.004    & 0.006932 & 0.010442 & 0.002787         & 0.005501               \\
%     0.01     & 0.006071 & 0.009468 & 0.001988         & 0.004656               \\
%     0.04     & 0.003758 & 0.006939 & 0.000993         & 0.002858               \\
%     0.1      & 0.002836 & 0.006082 & 0.000736         & 0.001967               \\
%     0.4      & 0.004895 & 0.006031 & 0.000443         & 0.000906               \\
%     1        & 0.006755 & 0.006996 & 0.000224         & 0.000393               \\
%     4        & 0.006019 & 0.00473  & 0.000364         & 0.000214               \\
%     \hline
% \end{tabular}

% \vspace{0.5cm}
% Test results for trajectories (unseen during training) with $\theta \in \theta_{ft}$ (unseen parameters) after pre-training but before finetuning.

% \vspace{0.2cm}
% \begin{tabular}{>{\centering\arraybackslash}p{0.10\linewidth}|>{\centering\arraybackslash}p{0.12\linewidth}|>{\centering\arraybackslash}p{0.12\linewidth}|>{\centering\arraybackslash}p{0.12\linewidth}|>{\centering\arraybackslash}p{0.12\linewidth}}
%     \hline
%     $\theta$ & $traj$     & $traj + t$ & $traj + t + param$ & $traj + t + param + fft$ \\
%     \hline
%     0.002    & 0.007243 & 0.010789 & 0.003189         & 0.005824               \\
%     0.02     & 0.004999 & 0.008276 & 0.001384         & 0.003741               \\
%     0.2      & 0.003433 & 0.005236 & 0.000597         & 0.001435               \\
%     2        & 0.006774 & 0.00631  & 0.002776         & 0.000827               \\
%     \hline
% \end{tabular}

% \begin{table*}[h]
%     \centering
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{@{}c|cccccccc|c|cccc|c@{}}
%     \toprule
%     \multicolumn{1}{l}{} & \multicolumn{9}{|c|}{\textbf{in domain $\Theta$}} & \multicolumn{5}{c}{\textbf{out of domain $\Theta$}} \\
%     \midrule
%     \textbf{$\theta$} & \textbf{0.001} & \textbf{0.004} & \textbf{0.01} & \textbf{0.04} & \textbf{0.1} & \textbf{0.4} & \textbf{1} & \textbf{4} & \textbf{id-mean} & \textbf{0.002} & \textbf{0.02} & \textbf{0.2} & \textbf{2} & \textbf{ood-mean} \\
%     traj & 7.39E-03 & 6.93E-03 & 6.07E-03 & 3.76E-03 & 2.84E-03 & 4.90E-03 & 6.76E-03 & 6.02E-03 & 5.58E-03 & 7.24E-03 & 5.00E-03 & 3.43E-03 & 6.77E-03 & 5.61E-03 \\
%     traj + t & 1.09E-02 & 1.04E-02 & 9.47E-03 & 6.94E-03 & 6.08E-03 & 6.03E-03 & 7.00E-03 & 4.73E-03 & 7.70E-03 & 1.08E-02 & 8.28E-03 & 5.24E-03 & 6.31E-03 & 7.65E-03 \\
%     traj + t + param & 3.64E-03 & 3.01E-03 & 2.18E-03 & 1.03E-03 & 6.16E-04 & 2.87E-04 & 1.31E-04 & 1.77E-04 & 1.38E-03 & 3.43E-03 & 1.52E-03 & 4.25E-04 & 1.89E-03 & 1.82E-03 \\
%     traj + t + param + fft & 5.98E-03 & 5.50E-03 & 4.66E-03 & 2.86E-03 & 1.97E-03 & 9.06E-04 & 3.93E-04 & 2.14E-04 & 2.81E-03 & 5.82E-03 & 3.74E-03 & 1.44E-03 & 8.27E-04 & 2.96E-03 \\ 
%     \bottomrule
%     \end{tabular}%
%     }
%     \caption{}
%     \label{tab:channels}
% \end{table*}

\begin{table*}[h]
    \centering
    \begin{tabular}{@{}ccc|cc|cc@{}}
    \toprule
    \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textbf{Burgers}} & \multicolumn{2}{|c|}{\textbf{Advection}} & \multicolumn{2}{c}{\textbf{Navier Stokes}} \\ \midrule
    & id-mean & ood-mean & id-mean & ood-mean & id-mean & ood-mean \\
    traj & 5.58E-03 & 5.61E-03 &  &  &  &  \\
    traj + t & 7.70E-03 & 7.65E-03 &  &  &  &  \\
    traj + t + param & 1.38E-03 & 1.82E-03 &  &  &  &  \\ \bottomrule
    \end{tabular}%
    \caption{\textbf{Input channels ablation:} In this experiment we try to see if all the channels of information provided to the model are truly required for best performance.}
    \label{table:channels-v2}
\end{table*}

==> src/experiments/tables/scaling-data.tex <==
% Test results for trajectories (unseen during training) with $\theta \in \theta_{pt}$ (seen parameters) after pre-training but before finetuning with increasing model size.

% \begin{tabular}{c|c|c|c}
%     \hline
%     $\theta$ & 50 traj per $\theta$ & 100 traj per $\theta$ & 200 traj per $\theta$ \\
%     \hline
%     0.001    & 0.010779             & 0.007389              & 0.003404              \\
%     0.004    & 0.00996              & 0.006932              & 0.002787              \\
%     0.01     & 0.008584             & 0.006071              & 0.001988              \\
%     0.04     & 0.004823             & 0.003758              & 0.000993              \\
%     0.1      & 0.002684             & 0.002836              & 0.000736              \\
%     0.4      & 0.001329             & 0.004895              & 0.000443              \\
%     1        & 0.000623             & 0.006755              & 0.000224              \\
%     4        & 0.001147             & 0.006019              & 0.000364              \\
%     \hline
% \end{tabular}

% \vspace{0.5cm}
% Test results for trajectories (unseen during training) with $\theta \in \theta_{ft}$ (unseen parameters) after pre-training but before finetuning.

% \vspace{0.2cm}
% \begin{tabular}{c|c|c|c}
%     \hline
%     $\theta$ & 50 traj per $\theta$ & 100 traj per $\theta$ & 200 traj per $\theta$ \\
%     \hline
%     0.002    & 0.010473             & 0.007243              & 0.003189              \\
%     0.02     & 0.006887             & 0.004999              & 0.001384              \\
%     0.2      & 0.001862             & 0.003433              & 0.000597              \\
%     2        & 0.000731             & 0.006774              & 0.002776              \\
%     \hline
% \end{tabular}


% \begin{table*}[]
%     \centering
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{@{}c|cccccccc|c|cccc|c@{}}
%     \toprule
%     \multicolumn{1}{l}{} & \multicolumn{9}{|c|}{\textbf{in domain $\Theta$}} & \multicolumn{5}{c}{\textbf{out of domain $\Theta$}} \\
%     \midrule
%     \textbf{$\theta$} & \textbf{0.001} & \textbf{0.004} & \textbf{0.01} & \textbf{0.04} & \textbf{0.1} & \textbf{0.4} & \textbf{1.0} & \textbf{4.0} & \textbf{id-mean} & \textbf{0.002} & \textbf{0.02} & \textbf{0.2} & \textbf{2.0} & \textbf{ood-mean} \\
%     50 & 1.14E-02 & 1.06E-02 & 9.32E-03 & 5.50E-03 & 3.14E-03 & 1.54E-03 & 5.68E-04 & 1.45E-03 & 5.44E-03 & 1.11E-02 & 7.64E-03 & 2.16E-03 & 5.22E-04 & 5.36E-03 \\
%     100 & 7.39E-03 & 6.93E-03 & 6.07E-03 & 3.76E-03 & 2.84E-03 & 4.90E-03 & 6.76E-03 & 6.02E-03 & 5.58E-03 & 7.24E-03 & 5.00E-03 & 3.43E-03 & 6.77E-03 & 5.61E-03 \\
%     150 & 4.41E-03 & 3.85E-03 & 3.00E-03 & 1.63E-03 & 1.13E-03 & 5.30E-04 & 2.11E-04 & 1.04E-04 & 1.86E-03 & 4.22E-03 & 2.20E-03 & 8.18E-04 & 8.63E-04 & 2.03E-03 \\
%     200 & 3.64E-03 & 3.01E-03 & 2.18E-03 & 1.03E-03 & 6.16E-04 & 2.87E-04 & 1.31E-04 & 1.77E-04 & 1.38E-03 & 3.43E-03 & 1.52E-03 & 4.25E-04 & 1.89E-03 & 1.82E-03 \\
%     300 & 2.77E-03 & 2.13E-03 & 1.35E-03 & 4.72E-04 & 5.32E-04 & 2.52E-04 & 1.23E-04 & 2.86E-05 & 9.58E-04 & 2.55E-03 & 7.42E-04 & 5.20E-04 & 3.42E-03 & 1.81E-03 \\
%     400 & 2.25E-03 & 1.63E-03 & 9.75E-04 & 3.34E-04 & 2.56E-04 & 9.25E-05 & 4.77E-05 & 2.49E-05 & 7.01E-04 & 2.01E-03 & 5.72E-04 & 2.40E-04 & 2.55E-03 & 1.34E-03 \\
%     500 & 2.30E-03 & 1.58E-03 & 8.58E-04 & 2.86E-04 & 1.58E-04 & 8.41E-05 & 5.17E-05 & 5.77E-05 & 6.72E-04 & 2.01E-03 & 4.62E-04 & 1.76E-04 & 1.88E-03 & 1.13E-03 \\ 
%     \bottomrule
%     \end{tabular}%
%     }
%     \caption{Scaling with data: each row shows the number of trajectories per in domain $\theta$ that the ViT has been trained on.}
%     \label{tab:scaling-data}
% \end{table*}

    \begin{figure*}[] 
        \centering
        \begin{minipage}{0.4\textwidth}
            \includegraphics[width=\linewidth]{src/experiments/images/id-trajectory-scaling.png}
            \caption{\textbf{In-Domain Scaling with more data}: The above plot shows how the prediction MSE varies with an increase in the training dataset size (i.e. the number of trajectories per parameter value $\omega$). We observe that the prediction error decreases steadily with an increase in the dataset size.             %\varun{2d-cfd numbers need to be redone}
            }
            \label{fig:scaling-data-id}
        \end{minipage}\hfill 
        \begin{minipage}{0.4\textwidth}
            \includegraphics[width=\linewidth]{src/experiments/images/ood-trajectory-scaling.png}
            \caption{\textbf{Out-of-Domain Scaling with more data}: The above plot shows how the prediction MSE varies with an increase in the training dataset size (i.e. the number of trajectories per parameter value $\omega$). We observe that the prediction error decreases steadily with an increase in the dataset size. 
            %\varun{weird advection 100 trajectories result?}
            }
            \label{fig:scaling-data-ood}
        \end{minipage}
    \end{figure*}

==> src/experiments/tables/scaling-model-size.tex <==
% \vspace{0.5cm}
% Test results for trajectories (unseen during training) with $\theta \in \theta_{pt}$ (seen parameters) after pre-training but before finetuning with increasing model size.

% \vspace{0.2cm}
% \begin{tabular}{c|c|c|c}
%     \hline
%      $\theta$ & L=2, H=128 & L=4, H=256 & L=8, H=512   \\
%      \hline
%      0.001 & 0.007245 & 0.003404 &  \\
%      0.004 & 0.006605 & 0.002787 &  \\
%      0.01  & 0.005506 & 0.001988 &  \\
%      0.04  & 0.003034 & 0.000993 &  \\
%      0.1   & 0.002100 & 0.000736 &  \\
%      0.4   & 0.001241 & 0.000443 &  \\
%      1.0   & 0.000629 & 0.000224 &  \\
%      4.0   & 0.000145 & 0.000364 &   \\
%      \hline
% \end{tabular}

% \vspace{0.5cm}
% Test results for trajectories (unseen during training) with $\theta \in \theta_{ft}$ (unseen parameters) after pre-training but before finetuning.

% \vspace{0.2cm}
% \begin{tabular}{c|c|c|c}
%     \hline
%     $\theta$ & L=2, H=128 & L=4, H=256 & L=8, H=512 \\
%     \hline
%     0.002    & 0.007032   & 0.003189   &                                \\
%     0.02     & 0.004243   & 0.001384   &                                \\
%     0.2      & 0.001752   & 0.000597   &                                \\
%     2        & 0.0013     & 0.002776   &                                \\ 
%      \hline
% \end{tabular}

% \begin{table*}[b!]
%     \centering
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{@{}c|cccccccc|c|cccc|c@{}}
%     \toprule
%     \multicolumn{1}{l}{} & \multicolumn{9}{|c|}{\textbf{in domain $\Theta$}} & \multicolumn{5}{c}{\textbf{out of domain $\Theta$}} \\
%     \midrule
%     \textbf{$\theta$} & \textbf{0.001} & \textbf{0.004} & \textbf{0.01} & \textbf{0.04} & \textbf{0.1} & \textbf{0.4} & \textbf{1.0} & \textbf{4.0} & \textbf{id-mean} & \textbf{0.002} & \textbf{0.02} & \textbf{0.2} & \textbf{2.0} & \textbf{ood-mean} \\
%     L=2, H=128 & 3.64E-03 & 3.01E-03 & 2.18E-03 & 1.03E-03 & 6.16E-04 & 2.87E-04 & 1.31E-04 & 1.77E-04 & 1.38E-03 & 3.43E-03 & 1.52E-03 & 4.25E-04 & 1.89E-03 & 1.82E-03 \\
%     L=4, H=256 & 7.25E-03 & 6.61E-03 & 5.51E-03 & 3.03E-03 & 2.10E-03 & 1.24E-03 & 6.29E-04 & 1.45E-04 & 3.31E-03 & 7.03E-03 & 4.24E-03 & 1.75E-03 & 1.30E-03 & 3.58E-03 \\
%     L=8, H=512 &  &  &  &  &  &  &  &  &  &  &  &  &  & \\
%     \bottomrule
%     \end{tabular}%
%     }
%     \caption{\textbf{Scaling with model size}: In this experiment we observe how the prediction error varies as we increase the model size. L is the number of Transformer encoder layers, while H is the hidden dimension. Building on \cite{well-read-students}, the number of attention heads A is set to H/64.}
%     \label{tab:scaling-model-size}
% \end{table*}

% \begin{table*}[t!]
%     \centering
%     \begin{tabular}{@{}ccc|cc|cc@{}}
%     \toprule
%     \multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{Burgers}} & \multicolumn{2}{|c|}{\textbf{Advection}} & \multicolumn{2}{c}{\textbf{Navier Stokes}} \\ \midrule
%      & id-mean & ood-mean & id-mean & ood-mean & id-mean & ood-mean \\
%     100 & 5.58E-03 & 5.61E-03 &  &  &  &  \\
%     150 & 1.86E-03 & 2.03E-03 &  &  &  &  \\
%     200 & 1.38E-03 & 1.82E-03 &  &  &  &  \\
%     300 & 9.58E-04 & 1.81E-03 &  &  &  &  \\
%     400 & 7.01E-04 & 1.34E-03 &  &  &  &  \\
%     500 & 6.72E-04 & 1.13E-03 &  &  &  &  \\ \bottomrule
%     \end{tabular}%
%     \caption{\textbf{Scaling with model size}: In this experiment we observe how the prediction error varies as we increase the model size. L is the number of Transformer encoder layers, while H is the hidden dimension. Building on \cite{well-read-students}, the number of attention heads A is set to H/64.}
%     \label{table:scaling-model-size-v2}
% \end{table*}

\begin{figure*}[] 
    \centering
    \begin{minipage}{0.4\textwidth}
        \includegraphics[width=\linewidth]{src/experiments/images/id-model-scaling.png}
        \caption{\textbf{In-Domain Scaling with model size}: The above plot shows how the prediction MSE varies with an increase in the model size (i.e. the number of learnable parameters). We observe that the prediction error decreases steadily with an increase in the dataset size. 
        %\varun{2d-cfd numbers need to be redone}
        }
        \label{fig:scaling-model-id}
    \end{minipage}\hfill 
    \begin{minipage}{0.4\textwidth}
        \includegraphics[width=\linewidth]{src/experiments/images/ood-model-scaling.png}
        \caption{\textbf{Out-of-Domain Scaling with model size}: The above plot shows how the prediction MSE varies with an increase in the model size (i.e. the number of learnable parameters). 
        % We observe that the prediction error decreases steadily with an increase in the dataset size. 
        %\varun{weird advection 100 trajectories result?}
        }
        \label{fig:scaling-model-ood}
    \end{minipage}
\end{figure*}

==> src/related-works.tex <==
\section*{Related Work} 
    % Physics Informed Neural Networks (PINNs) \cite{PINN} have received a lot of attention in the scientific machine learning community. PINNs learn PDE solutions using a neural network based architecture by minimizing the residual. They have been shown to work well for trivial problems but struggle with more complex problems. % PINNs are also trained for a single PDE parameter/parameter set, i.e they need to be retrained for a different parameter/parameter set.

    
    % \begin{itemize}
    %     \item Finite-dimensional operators
    %     \item Neural operators: Neural Operator (OG), DeepONet, NO-2
    %     \item FNO, FNO-v2 
    %     \item Lie Symmetries 
    %     \item ViTO
    %     \item PolyMathic
    % \end{itemize}

    % \varun{Need to discuss a bit more here to formulate this clearly!}

    There has been a lot of interest in using machine learning methods to create neural solvers for PDEs \cite{Sirignano2018, Zang2020, Raissi2019} due to its various scientific and engineering applications. Recently, the idea of learning the solution operator has gained a lot of attention \cite{NO2023}.

    The learned solution operator can be a finite-dimensional operator \cite{FDO-1, FDO-2, FDO-3} that maps between finite dimensional Euclidean spaces or it can be classified as a neural operator \cite{NeuralOperator, DeepONet, NO-2} that learns mappings between function spaces. Finite dimensional operators are by definition mesh dependent whereas neural operators are grid invariant \cite{FNO}.
    
    Out of the many architectures used to build neural solvers, the Fourier Neural Operator (FNO) \cite{FNO} has shown to outperform most other deep learning methods over a variety of different systems \cite{PDEBench}. 

    While significant progress has been made towards building fast and efficient neural solvers, the majority of works in the field are still limited by the fact that the models are trained to solve for a fixed value of PDE parameters. These models are not amenable to change of PDE parameters without retraining the network from scratch. While some attempts have been made to solve this problem \cite{brandstetter2022message, cape, FMfluid}, neither of them use a transformer based architecture.
    
    Transformers are known to demonstrate strong scaling properties with data and model size \cite{gpt1, gpt2, gpt3}, making them the ideal candidate to build large foundation models. While this work does not claim to be a foundation model, the ability to generalize across PDE parameters is required for a scientific foundation model \cite{polymathic}, and thus motivate the choice of architecture. In particular, we choose to make use of a vision transformer \cite{vit}. 

    This work proposes a Vision Transformer based network that learns to solve a PDE over a parameter space, in essence learning a family of finite-dimensional operators that generalizes well to any value of PDE parameters. It should be noted that, like other finite-dimensional operator methods, our approach is mesh-dependent.

    While \cite{ViTOperator} has used a Vision transformer to create a neural solver it suffers from the same problem of only being applicable to a fixed set of PDE parameters.

    % \amal{define family of PDEs}.

    % We build on these methods by learning a more general network that can predict the solution for a family of PDEs (i.e. with different parameter values).

    % The Fourier Neural Operator (FNO)  has recently gained a lot of traction in the scientific machine learning community. FNOs essentially try to learn the solution operator, mapping the initial condition to the PDE solution at some time t. This is primarily achieved by taking convolutions in fourier space. FNOs learn the solution operator by being trained on input output pairs of the initial condition to the solution of the PDE for some fixed PDE parameters. Thus they are restricted to being able to predict solutions for a single parameter set.

    % While this work is considerably different from the FNO, we compare the performance of our method with the FNO as the FNO performs very strongly compared to other deep learning methods \cite{FNO}.

    % The main goal of this work is to be able to overcome this issue by proposing a model that allows one to learn a family of solution operators that can make accurate predictions on a parameter space.
